RelTransformer: A Transformer-Based Long-Tail Visual Relationship Recognition

The visual relationship recognition (VRR) task aims at understanding the pairwise visual relationships between interacting objects in an image. These relationships typically have a long-tail distribution due to their compositional nature. This problem gets more severe when the vocabulary becomes large, rendering this task very challenging. This paper shows that modeling an effective message-passing flow through an attention mechanism can be critical to tackling the compositionality and long-tail challenges in VRR. The method, called RelTransformer, represents each image as a fully-connected scene graph and restructures the whole scene into the relation-triplet and global-scene contexts. It directly passes the message from each element in the relation-triplet and global-scene contexts to the target relation via self-attention. We also design a learnable memory to augment the long-tail relation representation learning. Through extensive experiments, we find that our model generalizes well on many VRR benchmarks. Our model outperforms the best-performing models on two large-scale long-tail VRR benchmarks, VG8K-LT (+2.0% overall acc) and GQA-LT (+26.0% overall acc), both having a highly skewed distribution towards the tail. It also achieves strong results on the VG200 relation detection task. Our code is available at https://github.com/Vision-CAIR/RelTransformer.

==> vg200/relatedWork.tex <==

\begin{figure*}[t!]
\centering
\includegraphics[width=0.76\linewidth]
                  {Figure/main_architecture_crop.pdf}
\caption{The architecture of our RelTransformer. It comprises a multi-layer global-context and a relational encoder. We display the detailed operations from a relational encoding layer in the left, which include memory attention and meshed attention fusion modules.}
\label{fig:main_model}
\end{figure*}

\noindent \textbf{Visual Relationship Recognition.} Correct visual relation prediction requires having a comprehensive understanding of the image contents, which guides many successful works in the literature. Early works employ RNN models to construct a global context by aggregating the node and edge features via iterative message passing such as \cite{messagePassing,motifNet,vctree,li2017scene,permutationInvariant}. e.g.,  VCTree \cite{vctree} composes a dynamic tree structure to organize the object orders and apply TreeLSTM \cite{tai2015improved} to aggregate features. 
There are also several graph convolutional network (GCN) \cite{gcn} approaches \cite{graph-rcnn,attentiveRelNet,chen2019knowledge,subgraphSceneGeneration}, which attempt to learn different importance weights to the neighborhood nodes. Lin \textit{et al.} \cite{gpsNet} extend the graph attention to also capture the node-specific contextual information and encode the edge direction information. More recently, there is also emerging a Transformer-based approach \cite{rtn}, which models the pairwise interaction among nodes and edges in two separate Transformer networks. Our model differs from it mainly in two aspects: a) we have a different message-passing flow in which we specifically aggregate relation features from the relation-triplet and global-context information. b) We further design an effective memory attention module for augmenting the long-tail relation representation. 



% c) We apply a feature fusion function to attentively leverage local, global and memory features into to the relation.
% RVL-BERT \cite{chiou2021visual} treats the relation prediction task as a multi-modal learning and connect linguistic and visual representation of the relation triplet in the hidden space. 


% attentiveRelNet  2019.  graph-rcnn


% neural motif parse the scene
% VCTree parses the scene graph into a tree, and then employ a tree biLSTM to learn the features from the tree.
% rnn: Scene Graph Generation by Iterative Message Passing, which use rnn to iteratively pass the messages.
% GPS-NET: we propose a novel message passing module that augments the node feature with node-specific contextual information and encodes the edge direction information via a tri-linear model.
% graph self attention: Attentive Relational Networks for Mapping Images to Scene Graphs: The other module is a graph self-attention module introduced to embed a joint graph representation through assigning various importance weights to neighboring nodes.
% gcn networks: Graph R-CNN for Scene Graph Generation. 

% there are two transformer-based methods such as Relation Transformer Network and multi-modal transformers. stating the difference between our model and other models.


% 1) Message passing in a tree structure. use lstm
% 1) messaging passing under a scene graph structure
% 3) leverage the relation prediction with the language prior.
% 4) two transformer-based methods such as RTN and multi-modal transformer.







% Numerous VRR methods have been studied in the literature \cite{li2017vip,lsvru,messagePassing,vrd}
% Lu \textit{et al.} \cite{vrd} performed the visual relationship prediction using pretrained object detectors and the prior language knowledge from word2vec \cite{word2vec} features. This investigation inspired many subsequent studies \cite{motifNet, lsvru, zhang2019graphical, sceneGenerationFromObjPhrase, attentiveRelNet,graph-rcnn}, all of which relied on a pretrained object detector to distinguish the relationships. Li \textit{et al.} \cite{sceneGenerationFromObjPhrase} proposed to augment the relationship prediction from the region caption. Additionally, various approaches that focus on different architectures of information propagation have also been examined in \cite{graph-rcnn, motifNet, vctree}. We employ a transformer-based architecture for refinement of the features and also show its effectiveness over other architecture types.

% Moreover, some studies \cite{vctree, multiAgentSGG} have considered the graph attributes such as the edge direction and node priority in their modeling. 


% \cite{motifNet} proposed to incorporate the statistical information about the dataset during the pipeline and hence improving upon the implicit bias present in the dataset. \cite{lsvru} allows for the visual and language features of the subjects, objects and relations to be adapted into a common embedding space using a visual and language embedding sub-networks. In \cite{zhang2019graphical}, authors propose to use contrastive losses to further improve the margin between similar class instance prediction, while \cite{gpsNet} also propose to use a different architecture with transformer blocks for an efficient scene graph generation. 

\noindent \textbf{Long-Tail Visual Relationship Recognition.} Long-tail problem is very severe in visual relation recognition (VRR) \cite{lsvru,ltvrd,gpsNet}. There are mainly two approaching directions to alleviate this problem. The first one is semantically guided visual recognition. In this case, language models \cite{word2vec} are employed for zero-shot or few-shot recognition \cite{frome2013devise,norouzi2014zero}. There are also several VRR works \cite{lsvru,ltvrd,graph-rcnn,yu2017visual} using the language priors as a guidance to learn relation features, which can derive a better classification on long-tail classes. The second direction is to apply the strategies that have been designed for unbalanced object detection, including various class imbalance loss functions (e.g. weighted cross entropy, focal loss \cite{focalLoss}, equalization loss \cite{eql}), sampling strategies (e.g., under-sampling \cite{underSampling},  over-sampling \cite{overSampling} and class-balanced sampling \cite{balanceSampling}), data augmentation \cite{cutmix,ltvrd}, meta learning \cite{ha2016hypernetworks, wang2017learning}, counterfactual learning \cite{tang2020unbiased}, memory modules \cite{oltr} and decoupling methods \cite{decoupling}. In our long-tail VRR experiment, we also leverage the language models and many aforementioned long-tail strategies to better classify long-tail relation types. But we focus on understanding their collaborative effect with our message-passing mechanism and how they influence head and tail predictions.  
% We show that the advantage of these mechanisms gets more significant on tail classes. % on their collaborative effect with our messaging passing strategy.






% Note: in this paper we use “relation” to refer to what is
% also known as ‘predicate” in previous works, and “relationship” or “relationship triplet” to refer to a hsubject, relation,
% objecti tuple.



% to leverag the long-tail visual detection losses. 




% There are mainly two streams for long-tail visual relation recognition. The first is 

% Extensive works have investigated the long-tail relation problems in various domains during the past years \cite{oltr, bengio2015the, ouyang2016factors, eql, focalLoss, decoupling}. Several approaches, e.g. weighted cross entropy and focal loss \cite{focalLoss} are designed to assign more weight to the tail classes. Furthermore, many approaches involving meta learning \cite{ha2016hypernetworks, wang2017learning}, regularization \cite{cutmix}, sampling (e.g., under-sampling \cite{underSampling},  over-sampling \cite{overSampling} and class-balanced sampling \cite{balanceSampling}), counterfactual learning \cite{tang2020unbiased}, memory modules \cite{oltr} and decoupling methods \cite{decoupling} have been proposed. In contrast to this, we propose using multi-context features and show its effectiveness for solving this problem. 







% In \cite{oltr}, the authors design a dynamic visual memory module along with modulated attention to encourage the generalization of tail classes. Kang \textit{et al.} \cite{decoupling} propose to decouple  the learning procedure into representation learning and classification and they show promising improvement. Tang \textit{et al.} \cite{tang2020unbiased} demonstrate that long-tail bias can be reduced by their proposed counterfactual causality. 




% \noindent \textbf{Transformers} Transformers \cite{vaswani2017attention} have been successfully applied in the field of natural language processing \cite{bert, gpt3} in the past few years. It is now gradually extended into many other domains including vision, biology and chemistry \cite{igpt,imageTransformer, visualgpt, biobert,chemistryTransformer,clinicalbert}. Transformer has the advantages of fast training speed, long-range dependency \cite{transformerxl,adaptiveAttentionSpan} and strong generalization ability with a large amount of training data \cite{bert, gpt3} compared to conventional language models such as LSTM \cite{lstm}. With this in mind, we decide to adapt transformers into the VRR setting.


% In our work, unlike previous VRR methods, we design a Transformer-based model and rely on various attention modules to explicitly aggregate the local, global and dataset-level features into the relation learning. Unlike the previous long-tail classification methods, our model is able to generate more discriminative long-tail relation representation by leveraging richer context features.  










% In \cite{parmar2018image}, authors propose to use transformer architecture to improve upon the classical image classification problem, while at the same time also apply it various on tasks such as super-resolution and generative modelling. To even further the roots of transformers in vision related tasks, \cite{carion2020end} use transformers for solving object detection and panoptic segmentation,  with the whole framework being end-to-end and also the first one to successfully incorporate the transformers as central building block in the pipeline. We propose a new transformer-based model called RelTransformer, which can be applied to one of longest standing problem in vision of relationship detection.


